Visualizing MuZero Models

MuZero, a model-based reinforcement learning algorithm that uses a value equivalent dynamics model, achieved state-of-the-art performance in Chess, Shogi and the game of Go. In contrast to standard forward dynamics models that predict a full next state, value equivalent models are trained to predict a future value, thereby emphasizing value relevant information in the representations. While value equivalent models have shown strong empirical success, there is no research yet that visualizes and investigates what types of representations these models actually learn. Therefore, in this paper we visualize the latent representation of MuZero agents. We find that action trajectories may diverge between observation embeddings and internal state transition dynamics, which could lead to instability during planning. Based on this insight, we propose two regularization techniques to stabilize MuZero's performance. Additionally, we provide an open-source implementation of MuZero along with an interactive visualizer of learned representations, which may aid further investigation of value equivalent algorithms.

==> Chapters/abstract.tex <==
AlphaZero has shown what model-based reinforcement learning is capable of when a perfect model of the environment is available.  Many recent approaches learn an abstract dynamics model end-to-end; MuZero has recently achieved this impressive feat both in board games and in Atari, utilizing  \emph{Value-Equivalence} to ensure that the reward trajectories within the abstract model are close to the reward trajectories within the environment. We have built a visualizer to  better understand the dynamic interplay of planning and abstract models and to see how learned values trace observed values. We report how visual intuition regarding abstract model learning can yield insights for improving the stability and learning of the algorithm. In particular, we found two methods for regularizing MuZero's transition function that showed potential in achieving this goal. %As the complexity of model-based reinforcement learning grows, so must the power of the tools that help us understand our models.

==> Chapters/background.tex <==


We will briefly recall salient details of the MuZero algorithm, based on \cite{schrittwieser_mastering_2020}. MuZero tackles deterministic MDPs (like Chess or Atari) denoted by a tuple $\langle \mathcal{S}, \mathcal{A}, \mathcal{T}, U, \gamma \rangle$. These represent the set of states, the set of actions, the mapping from state-action pairs to new states, the mapping from state-action pairs to rewards, and the discount factor, respectively \cite{sutton_reinforcement_2018}. %Discounting of rewards is used to ensure convergence of the cumulative reward in non-finite MDPs; larger values for $\gamma$ increase the influence of distant rewards on our learning agent. 
Internally, MuZero defines an abstraction over $\mathcal{S}$ and the state transition and reward functions, which we denote as the learned MDP tuple $\langle \latentS, \mathcal{A}, \widetilde{\mathcal{T}}, R, \gamma \rangle$---we interchangeably refer to the learned MDP as the abstract or latent MDP.

\begin{figure}%{r}{0.35\textwidth}
\centering
    \includegraphics[width=.65\linewidth]{Figures/MuZeroMCTS.pdf}
    \caption{Illustration of MuZero's RNN unfolding during MCTS. During training, actions are given by the data.} \label{fig:background:MuMCTS} %\vspace{-3em}
\end{figure}

MuZero consists of three distinct neural networks, namely the state embedding function $h_\theta$, the dynamics function $g_\theta$, and the prediction network $f_\theta$. The embedding function maps the real MDP's state space to a starting state in the abstract MDP's state space, $h_\theta: \mathcal{S} \rightarrow \latentS$ where $\latentS \subseteq \mathbb{R}^{\dim(h_\theta)}$. The dynamics function $g_\theta$ represents an environment model $\model = \langle \widetilde{\mathcal{T}}, R \rangle$ for the abstract MDP, enabling look-ahead search. States provided by the model $\model$ are passed to the prediction network, which outputs a prediction of the action-selection distribution and the state value function, $f_\theta: \latentS \rightarrow \langle \mathcal{P}(\mathcal{A}) , \mathbb{R} \rangle$, where $\mathcal{P}(\mathcal{A})$ denotes the space of probability distributions over $\mathcal{A}$. We individually denote the predictions by $f_\theta$ as $\textbf{p}^k_t$ and $V^k_t$, respectively---we utilize subscripts to index time in the real environment and superscripts to index time in the learned environment. Putting this together, MuZero concatenates its three neural networks into a one-to-many Recurrent Neural Network (RNN) that can be recursively unfolded for planning.

MuZero performs planning using AlphaZero's MCTS inside the RNN model $\model$. Figure \ref{fig:background:MuMCTS} illustrates this procedure at the top level. Based on a trajectory of state observations $o_1, \dots, o_t$, the embedding network $h_\theta$ yields a starting state for the abstract MDP $\latents^0_t$. Then, given some action $a^0$, MuZero recurrently expands new nodes within the search tree using the dynamics network $\langle \latents_t^1, r_t^1 \rangle = g_\theta(\latents_t^0, a^0)$. The tree expansion is governed by the prediction network $f_\theta$ and an upper confidence bound to balance exploration and exploitation \cite{silver_general_2018, rosin_multiarmed_2011}. Each MCTS call aims to generate improved estimates of the root-level predictions $\textbf{p}^0_t$ and $V^0_t$. These tree search statistics, $\pi_t, \nu_t \sim \mathrm{MCTS}(o_1, \dots, o_t; \mu_\theta)$, are used for action sampling and learning targets. 

Through general game playing or self-play, MuZero collects trajectories of MCTS statistics, performed actions in the real MDP, and observations of states and rewards. As the three neural networks are connected end-to-end as an RNN, the entire model $\mu_\theta = (h_\theta, g_\theta, f_\theta)$ can be trained jointly with error gradients from $f_\theta$ and $g_\theta$ under the following loss \cite{silver_general_2018, schrittwieser_mastering_2020}:
\begin{equation}\label{eq:background:loss}
\begin{split}
    l(\theta) = & \sum^K_{k=0} l^r(u_{t+k}, r^k_t) + l^v(z_{t+k}, V^k_t) + \\
    & l^p (\pi_{t+k}, \textbf{p}_t^k) + \lambda \|\theta\|^2_2,
    \end{split}
\end{equation}
where $l^r=0$ for $k=0$. The backed up value $z_t$ is either an $n$-step TD-return using the MCTS value as the bootstrap target $z_t = \sum^{n}_{i=1} \gamma^{i-1} u_{t+i} + \gamma^n \nu_{t+n}$ or the Monte-Carlo return for boardgames \cite{sutton_reinforcement_2018}. The loss functions for each prediction are generic cost functions such as cross-entropy or squared error, left transparent to the utilized encoding. Finally, the loss includes L2 regularization on $\theta$ governed by the scalar $\lambda$. It becomes apparent that this algorithm becomes equivalent to AlphaZero when $K=0$ and the parameters for $g_\theta$ and $h_\theta$ are frozen. 

% Move to appendix:?
As a final note, MuZero accommodates MCTS for environments with arbitrary reward scaling by min-max normalization of edge-values within the P-UCT formula \cite{schrittwieser_mastering_2020, rosin_multiarmed_2011}. The normalization statistics for this are freshly accumulated at each step in the real MDP (during each individual MCTS procedure), eliminating the need for \emph{ad-hoc} reward transformations. This trick can also be transferred to AlphaZero, enabling both algorithms to handle generic deterministic MDPs. For a broader overview on the large amount of detail underlying MuZero, we refer the reader to the supplementary material accompanying
\cite{schrittwieser_mastering_2020}.

==> Chapters/conclusion.tex <==
In this work we developed an approach for visualizing learned representations by MuZero to provide intuition behind the algorithm's learning process and state-abstraction. Based on these insights, we demonstrated that introducing regularization penalties to the MuZero agent, derived from a geometric interpretation of the learned MDP, can aid stability and reliability of learned models. 
Several works report on the success of abstract model approaches in model-based reinforcement learning, where  abstract internal representations are learned and used for planning \cite{hafner2019dream,hafner2020mastering,kaiser2019model,ha2018world,babaeizadeh2020models,ermolov2020latent}. Understanding the training processes of abstract representations is challenging, and we hope that 
%An interesting trend in recent reinforcement learning is to refer to agents that plan within, or learn, an MDP model of the environment as `latent' or `imaginary' models. Analogously to complex numbers, these models are not imaginary and naturally extend AlphaZero to end-to-end model learning. We hope that 
our work sheds insight, and in turn comprehension, into this family of algorithms as a means of aiding future research. 




==> Chapters/discussion.tex <==
The  MuZero algorithm is remarkably successful at solving and learning complex dynamics models of MDPs, and the results ar impressive \cite{schrittwieser_mastering_2020}. Our results indicate, however, that it may also be plagued by learning instability and unreliable results. Unfortunately, the large computational requirements prevented us from running statistically significant experiments on similarly large scale environments as reported in \cite{schrittwieser_mastering_2020}. 

Nevertheless, our results show that there are  benefits to including sources of regularization for shaping learned MDP models within MuZero. In particular we found that a contrastive regularization term can aid reliability of the learned MDP for planning with sparse observations; future work could investigate how this would translate to applying MuZero in partially observable environments. 

We believe that one of the main causes for instability in MuZero is the initialization of the agent networks, the initial representation can potentially define a highly degenerate MDP model. Given a reward-dense environment, this may not pose  too large of a problem, however it can lead to swift overspecialization in sparse reward environments due to the use of bootstrapping. This  corroborates the arguments of representation learning in deep reinforcement learning by \cite{dabney_valueimprovement_2020} and empirical findings by \cite{van_seijen_loca_2020}. The latter showed how local pre-training based on a performance metric improved MuZero's learning speed considerably. Our conjecture is that such a form of pre-training allows the internal MDP to more rapidly take a non-degenerate shape near reward salient areas. This in turn can improve the efficacy of bootstrapping. To confirm this, future work can track a density map of the agent's trajectories within the learned and real environment, this could also indicate how MuZero explores within the learned and real environment and whether it gets routinely stuck within parts of its model.  

We consider the insights yielded by our visualization system to be the main contribution of our work, and it is visually pleasing to observe how MuZero learns and settles on its abstract MDP model. As indicated by the value map contours, we found that the embedding function groups environment observations based on their on-policy value function estimate. In other words, adjacent points within the learned MDP model often have similar reward prospects in the actual environment, confirming their Value Equivalence. For future work, it would also be interesting to investigate learned representations by MuZero where the dimensionality of the learned MDP is lower or equal to the environment. 

Furthermore, we found a pattern that the learned models maximally spread states according to their value estimate. This can be observed most clearly in the embedding on the right of Figure \ref{fig:results:embedding:mountaincar}. The dark and light contours are almost  linearly interpolated following the axis of most variance---this pattern occurred in all of our trained agents. This pattern could indicate how the planning procedure moves throughout the model and what kind of function the dynamics network represents. It could also mean that MuZero's value function learns a simple linear pattern within the learned space and that learning of the environment's value landscape is mostly performed by the dynamics and embedding functions. Future work should investigate this relation further and how this could be visualized in terms of the dynamics function instead of the embedding.

% Add later?: Areas of high reward and low reward seem maximally separated, this may give an indication of why planning works. MuZero's dynamics seem to be able to plan over reward preferences (it does not have to rely on a root-level prediction as it can step forward throughout its model to evaluate multiple preferenes and arrive at a final decision.

% Add discussion: Density of data for observations and points within the learned space to visualize how the agent explores within both spaces.

% Add discussion: Dynamics upon refresh jumps back to original trajectory.


==> Chapters/intro.tex <==
% Muzero is new state of the art model based RL algorithm
% Plans on a learned model
% unclear what the learned model represents, not much research in understanding this

Model-based reinforcement learning has shown remarkable success in learning complex control tasks, as illustrated by the AlphaZero and MuZero algorithms \cite{silver_mastering_2017, silver_general_2018, schrittwieser_mastering_2020}, combining Monte Carlo Tree Search planning \cite{browne2012survey}  and deep residual networks. The premise of look-ahead search is to more effectively evaluate the future impact of possible actions; AlphaZero cleverly uses this to sample strong action-selection policies that simultaneously serve as effective learning targets. However, performing look-ahead search necessitates a mechanism to extrapolate current states into the future. For the board games of AlphaZero, the game rules provide  a perfect simulation of the environment. In most real-world problems no such perfect dynamics model is available \cite{silver_general_2018, silver_mastering_2017}. While it is possible to learn a Markov Decision Process (MDP) model of an environment,  approximations of state-transitions often result in large compounded errors when planning over long horizons \cite{sutton_reinforcement_2018, schrittwieser_mastering_2020, oh_value_2017}. 

Many recent model-based reinforcement learning approaches perform end-to-end learning of the MDP with abstract representations of states and values \cite{silver_predictron_2017,schrittwieser_mastering_2020,oh_value_2017}. Grimm et al.\ introduced the \emph{Value Equivalence} principle \cite{grimm_value_2020}, explaining the success of abstract models through a focus on values, instead of detailed modeling of an MDP's transition dynamics. This principle is behind the empirical success of MuZero  \cite{schrittwieser_mastering_2020}, which hybridizes Value Prediction Networks (VPNs) \cite{oh_value_2017} and the AlphaZero algorithm \cite{silver_general_2018}. MuZero plans over a learned MDP, taking the form of an unrolled Recurrent Neural Network (RNN), where action trajectories yield equivalent rewards in both the environment and in the learned MDP. The learned MDP consists of abstract states, values, and rewards; state-transitions within the learned MDP convey no semantic meaning with respect to the real MDP.

As a result of relaxing state-transitions in the learned MDP, the MuZero agent can learn to generalize over portions of the state-space with similar \emph{on-policy state values}. However, this also further extends AlphaZero's black-box, which could make planning seem obfuscated from an outside perspective. To make this process more tangible, we have re-implemented MuZero to be able to visualize the learned representations and to provide intuition on how MuZero achieves abstraction over an environment and its dynamics. We achieve this through (interactive)  visualization of \emph{Value Equivalence} in low dimensional settings. Based on this, we demonstrate how to influence the  properties of the learned MDP by  varying terms in the loss function. 
The contributions of this paper are as follows:
\begin{itemize}
    \item MuZero's abstract models build representations that may be far from the environment; we built a visualizer to better understand the dynamic abstract representations of states, policies, and rewards 
    \item The visualizer allows the study 
    %the principle of value equivalence in action, 
    a complicated end-to-end learning process involving an MCTS planner and three abstract models
    \item We find two regularization methods to improve the stability of the learning process of MuZero 
\end{itemize}
%The visualizer provides a look into the ``brain" of MuZero.




==> Chapters/methods.tex <==
In this section we present a practical example of visualizing MuZero as depicted in Figure \ref{fig:understanding:abstraction}, along with quantifying the effects of the transition function regularization methods from Figure \ref{methods:fig:regularization} on the learned MDP's semantics. We measured the stability of learning in terms of reward progression and we measured the reliability of learned models in terms of trials rewards when acting \emph{strictly} within the learned model. We complemented this with a hyperparameter analysis over various loss and model properties for investigating general stability and reliability of the algorithm. As MuZero incurs an overhead in learning due to added complexity of learning an MDP model, we compared MuZero's performance to AlphaZero agents with perfect environment models. We provide a complete reimplementation of MuZero based on the original paper \cite{schrittwieser_mastering_2020} along with an adaptation of AlphaZero for single-player domains \cite{silver_general_2018} in Python and Tensorflow 2.0 \cite{tensorflow2015-whitepaper}. Our code follows the AlphaZero-General framework \cite{nair_suragnairalpha} and is available at \url{https://anonymized.org}, %\url{https://github.com/kaesve/muzero}, 
along with resulting data.

\begin{table*}[h]
    \centering
    \renewcommand{\arraystretch}{1.1}
    \caption{Overview of the hyperparameter grid that we used to ran experiments. We repeated the Cartpole runs $r=8$ times; MountainCar agents were only run $r=1$ time. Color annotations correspond to the loss regularization methods depicted in Figure \ref{methods:fig:regularization}.}
    \begin{tabular}{p{3.8cm}|l|l}
         Hyperparameters & CartPole & MountainCar \\
         \hline
         RNN Unroll steps $K$ & $\{1, 5, 10\}$ & $3$ \\
         RNN Neurons $L$ & $\{4, 8\}$ & $\{4, 8\}$ \\
         Transition Regularization & $\{\mathrm{None}, \textcolor{encoder}{D_{KL}(h_\theta \vert\vert g_\theta)}, \textcolor{decoder}{h^{-1}_\theta}\}$ & $\{\mathrm{None}, \textcolor{encoder}{D_{KL}(h_\theta \vert\vert g_\theta)}, \textcolor{decoder}{h^{-1}_\theta}\}$ \\
         Regularization Strength $\omega$ & $\{0.01, 0.1, 1\}$ & $1$ \\
    \end{tabular}
    \label{tab:methods:parameters}
\end{table*}

For lucidity, we performed experiments on low dimensional classical control environments from OpenAI's gym \cite{openai_gym}. Our main experiments were run on the MountainCar environment. We utilized MuZero's canonical loss along with the decoding and contrastive regularization terms using $\omega = 1$, as explained in the previous section. For the contrastive loss we minimized the relative entropy from $g_\theta$ to $h_\theta$, for the decoding loss we minimized the mean square error between decoded observations $h^{-1}_\theta$ and true observations. We developed an interactive visualization tool for investigating learned MuZero models on the MountainCar environment at \url{https://anonymized.org}.\footnote{Video in supplemental material} %\url{https://kaesve.nl/projects/muzero-model-inspector/}. 
We encourage the reader to play around with this tool as we personally found this to provide more insight than static $2$-dimensional images. See also the \href{ap:supplementary_figures}{Appendix} for additional visualizations.

We investigated the overall stability of learning by performing a hyperparameter analysis on the CartPole environment. We varied hyperparameters that have direct influence on the learning of MuZero's internal MDP, such as the number of unroll steps $K$ and the latent dimensionality $L$, using the factorial experimental design from Table \ref{tab:methods:parameters}. Appendix \ref{ap:parameters} provides all other parameters and network designs. For each hyperparameter configuration we measured the configuration's empirical success ratio over $r=8$ repetitions. This ratio denotes whether the agent was able to consistently solve the MDP during training evaluated over $n=10$ episodes and a greedy MCTS visit count temperature $\tau = 0$. 

To measure the reliability of learned models, we measured the cumulative reward in the \emph{real MDP} when acting fully within the \emph{learned MDP}. We achieved this by generating action trajectories within the learned model for $x$ time steps before grounding the agent again by encoding the real MDP state with $h_\theta$ --- i.e., by blindfolding the agent and only providing environment observations periodically \cite{freeman_learning_2019}. The cumulative rewards for these episodes were averaged over $20$ runs and are supposed to give an indication of how far the learned MDP model diverges from the real MDP.

All experiments were run on the CPU. The hyperparameter analysis experiment was run asynchronously on a computing cluster using 24 threads at 2GHz. All MountainCar runs were run sequentially on a laptop with a 9th generation i7 CPU. All runs could be completed in approximately one week. On average it took about half a day to train an agent on any particular environment.


==> Chapters/related.tex <==
Visualizing deep networks to understand loss functions and the general functioning of the learning processes has a long history, see for example \cite{bischof1992visualization,yosinski2015understanding,karpathy2015visualizing,li2018visualizing}. 

We focus on understanding a new class, abstract models in reinforcement learning, and specifically on MuZero. 
The MuZero algorithm displayed remarkable success for performing action planning without access to a perfect transition model by learning abstractions over an environment's state-space \cite{schrittwieser_mastering_2020}. MuZero models the real state space into abstract representations \cite{oh_value_2017} for states, values, and rewards, and plans on this compressed, abstract, space. Grimm et al.~\cite{grimm_value_2020} explain the success of MuZero and related approaches through the introduction of \emph{Value Equivalence principle}. They argue that the space of environments (or models) with equivalent reward dynamics is much larger than the space of environments with equivalent state transition and reward dynamics. Thus the efficiency of representation learning for an environment can be improved. Initial work in this area, the Predictron \cite{silver_predictron_2017}, focused on forward predictions of a shaped value function.  The Value Prediction Network (VPN) by \cite{oh_value_2017} extended work in this area to predict the generic MDP value, reward, and discount functions.

MuZero combines the MDP learning from VPNs with the value and policy learning of AlphaZero \cite{oh_value_2017, silver_mastering_2017, silver_general_2018}. MuZero's model learning includes the Monte Carlo Tree Search (MCTS) for sampling strong action policies and learning targets, the self-play for data generation, and the forward prediction of the value function and reward function. MuZero extends VPNs by including an action-selection policy in the forward predictions, but foregoes prediction of the discount function.  MuZero also incorporates  distributional deep Q-learning for effective reward function parameterization \cite{pohlen_observe_2018, kapturowski_recurrent_2018}, along with prioritized experience replay in non-adversarial settings \cite{schaul_prioritized_2016}. We explain the essence of the algorithm in the next section.

For any particular environment, the goal of MuZero is to learn a coordinate in the space of value equivalent models. Empirically, we found it difficult to predict how learning of MuZero would unfold---we found that the success of solving environments showed large variance depending on the utilized hyperparameters and random seeds. In order to identify potential issues during MDP learning and general algorithm configuration, reasonable intuition behind the learning process is invaluable. Visualization of the learned models can aid in this regard and potentially makes the learning process more tangible. For example, work by \cite{li_visualizing_2018} showed how visualizing the loss landscape of a neural network can indicate smoothness of an optimization criterion. Furthermore, \cite{szymanski_visualising_2011} illustrate how kernel-methods project lower dimensional data to higher dimensional spaces for classification. We remark that a common approach for visualizing neural network mappings are \emph{non-linear} dimensionality reduction techniques, such as Stochastic Neighbour Embedding \cite{hinton_stochastic_2002}. We focus instead on linear projections in low dimensional environments, as non-linear dimensionality reduction can significantly alter the semantics of learned MDP models.

% TODO: Kernel-projections and linear separability. DONE.


==> Chapters/understanding.tex <==
The loss function of MuZero (Equation \ref{eq:background:loss}) creates a form of contraction mapping akin to generalized policy iteration methods \cite{silver_general_2018, sutton_reinforcement_2018}; an improvement to the neural network predictions improves the tree search which in turn gives us further improved learning targets. As these gradients are also propagated throughout the MDP model, this causes the MDP to update its rules as to best predict the MCTS statistics and the reward function. This mechanism allows MuZero's networks to map arbitrary transformations as to best fit the reward landscape of the real MDP.

\begin{figure}[h]
    \centering
    \includegraphics[width=.9\linewidth]{Figures/MDP_Abstraction_example.pdf}
    \caption{Illustration of MuZero's MDP abstraction in a low dimensional hypothetical example. Given an identical sequence of actions, the path mapped by the dynamics function conflicts with the path mapped on the embedded trajectory observations. Despite this difference in the learned state-space (right), both trajectories yield equivalent results when applied in the real state-space (left). Note that the grid shown on both sides are somewhat deceptive as $h_\theta$ can be non-injective and non-surjective.}
    \label{fig:understanding:abstraction}
\end{figure}

This concept is illustrated in Figure \ref{fig:understanding:abstraction}, which visualizes a learned MuZero model operating in a low dimensional observed and learned state-space. The left figure illustrates an action and state-transition trajectory (black dotted line) through some real MDP together with the boundaries its 2D state-space. The right figure shows a hypothetical embedding of the real MDP's state-space along with the embedded state-transition trajectory produced by $h_\theta$ (blue dotted line). The state-space embedding defines a non-linear projection to a manifold inhabiting the abstract state-space. In Figure \ref{fig:understanding:abstraction} we see that this projection has a fold in euclidean space. Distant spatial coordinates (in euclidean space) within the real MDP may lie in relative adjacency inside the learned embedding. This could indicate that this part of the real MDP's state-space has similar reward values.
% Wat bedoel je met prosperity?
The behaviour of the learned transition function is depicted by the green dotted line, which shows the same \emph{action} trajectory from the real MDP but passed through MuZero's dynamics function given $\latents_t^0$. This trajectory shows % exemplifies 
Value Equivalence as the dynamics function detaches from the observation embeddings while achieving equivalent results to the embedded trajectory (blue) in terms of rewards in the real MDP.

For high-dimensional problems visualization becomes more difficult. Yet, it may still be possible to quickly identify practical issues such as transition degeneracy or misadapted embeddings through slicing (or linear projections). Non-linear dimensionality reduction techniques could also aid in this regard \cite{maaten2008visualizing}, however, these can also  alter the semantics of the learned functions. A better choice would be to project the abstract MDP to the principal component space from data by the dynamics function or the state-space embedding. Alternatively, we could slice the high dimensional state space based on (relative) entropy measures of data from these two functions.


\subsection{MDP Representation Shaping by Regularization}
In order to plan over reasonably long time horizons, a learned model must remain relatively congruent to reality when extrapolating into the future---at least in terms of Value Equivalence for MuZero \cite{grimm_value_2020}. One persistent issue in learning efficient representations for a MDP model is overfitting \cite{sutton_reinforcement_2018, dabney_valueimprovement_2020}, the use of bootstrapping amplifies this issue by overadapting to an agent's current inexperience. \cite{dabney_valueimprovement_2020} provide an insightful perspective on this for model-free methods and show how auxiliary loss functions can act as regularizers to the reward signal. We adopt this insight as a way of regularizing the MDP model learning to make it more stable and reliable.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{Figures/MuZeroDrawingCombined.pdf}
    \caption{Illustration for two methods to influence the geometric shape of MuZero's learned MDP model as depicted in Figure \ref{fig:understanding:abstraction}. The loss scheme at the top adds a contrastive loss to penalize the dichotomy between $h_\theta$ and $g_\theta$, the top-right figures illustrate that this forces the trajectory of $g_\theta$ to lie close to the trajectory of $h_\theta$. The bottom diagram illustrates adding a jointly trained neural network decoder $h^{-1}_\theta$ for the latent trajectories; this requires the learned MDP model to retain a degree of congruency with the real MDP's state-transition function. }
    \label{methods:fig:regularization}
\end{figure}

Aside from shaping the reward/value landscape, MuZero's learned representation can also be influenced through its transition model. As MuZero's representation is formed through the environment's reward landscape, it is possible that sparse rewards can cause degeneracy in the learned transition or embedding function; we observed similar phenomena upon random initialization. The reason is that observations with identical value function estimates or expected reward values, as given by the data, can be considered identical \cite{grimm_value_2020}. We can ameliorate overadaptation by imposing differentiable penalties based on divergence between the learned and real MDP. 

One solution  to this problem is to add a discrepancy penalty $l^{d}\left(h_\theta(s_{t+k}^0), g_\theta(s^k_t, a^k_t)\right)$ between the embedding and dynamics function to MuZero's loss (Equation \ref{eq:background:loss}) where its influence can be governed by a scalar $\omega$. This penalty enforces the transition function to lie close to the embedding function, which may be advantageous when the embedding is relatively well adapted. In order to prevent $h_\theta$ from adapting to $g_\theta$ we cancel incoming gradients for $h_\theta$ when $k>0$. This results in a form of contrastive loss often seen in Siamese Networks \cite{chen_exploring_2020, koch_siamese_2015}. 

A second approach to ensure that the embedding function and transition function do not collapse to trivial solutions is to use an AutoEncoding scheme \cite{goodfellow2016deep} . This ensures that MuZero retains a form of congruency with the real MDP's state transition function proportional to the regularization strength $\omega$. This can be achieved by introducing a fourth neural network serving as a latent-state decoder $h^{-1}_\theta(s_t^k) \rightarrow o'_{t+k}$ and complementing the loss (Equation \ref{eq:background:loss}) with a discrepancy function $l^d$ between decoded $h^{-1}_\theta(s_t^k)$ and observed future states $o_{t+k}$. This approach can be advantageous in initial stages of learning, as state transitions are often dense in information whereas reward signals may be sparse. This could aid exploration in early stages of learning but will ultimately not be necessary for learning strong control policies.

Both approaches can be visualized in terms of their computation graph and of their effect on the learned MDP's semantics as shown in Figure \ref{methods:fig:regularization}. If the dynamics function $g_\theta$ is ill-adapted, the contrastive penalty can enforce $g_\theta$ to lie close to $h_\theta$ as a means of reducing extrapolation. Its efficacy is dependent on the mapping defined by $h_\theta$, however, as learned transitions lie close to observation embeddings this may make the final MDP model more reliable. The second penalty is illustrated in the bottom row of Figure \ref{methods:fig:regularization}. This AutoEncoding scheme defeats the Value Equivalence principle to some degree but can allow the embedding to quickly take a non-trivial shape within the learned space.


==> experiments.tex <==
\begin{table}[!h]
    \centering
    \renewcommand{\arraystretch}{1.1}
    \caption{Overview of factorial experimental design: 1) regularization type, 2) regularization strength ($\omega$), 3) latent roll-out depth ($K$), and 4) latent dimensionality ($L = |\latents |$). Color annotations correspond to the loss regularization methods depicted in Figure \ref{methods:fig:regularization}.}
    \begin{tabular}{p{1.2cm}|p{2.9cm}|p{2.9cm}}
         Hyperpar. & CartPole & MountainCar \\
         \hline
         Regular. & $\{\mathrm{None},\textcolor{encoder}{\mathrm{Contr.}}, \textcolor{decoder}{\mathrm{Dec.}} \}$ & $\{\mathrm{None},\textcolor{encoder}{\mathrm{Contr.}}, \textcolor{decoder}{\mathrm{Dec.}} \}$ \\
         $\omega$ & $\{0.01, 0.1, 1\}$ & $\{1\}$ \\
         $K$ & $\{1, 5, 10\}$ & $\{3\}$ \\
         $L$ & $\{4, 8\}$ & $\{4, 8\}$ \\
    \end{tabular}
    \label{tab:methods:parameters}
\end{table}

We will now experimentally study our regularized versions of MuZero compared to standard MuZero. As an additional baseline, we also include an adaptation of AlphaZero for single-player domains \cite{silver_general_2018}, i.e., a similar agent with a perfect environment model. We provide a complete reimplementation of MuZero based on the original paper \cite{schrittwieser_mastering_2020}. All code is written in Python using Tensorflow 2.0 \cite{tensorflow2015-whitepaper}. The code follows the AlphaZero-General framework \cite{nair_suragnairalpha} and is available at \url{https://github.com/kaesve/muzero}, 
along with all resulting data. 

We tested our work on low-dimensional, classic control environments from  OpenAI's Gym \cite{openai_gym}, in particular CartPole and MountainCar. These are low-dimensional problems for which it is feasible to visualize and interpret the resulting model. We also developed an interactive visualization tool to visualize learned MuZero models on the MountainCar environment at \url{https://kaesve.nl/projects/muzero-model-inspector/#/}.\footnote{Please find a video of our tool in the supplementary material.}
We encourage the reader to play around with this tool as we personally found this to provide more insight than static $2$-D images.

All hyperparameters can be found in Appendix \ref{ap:parameters} in supplemental material. For the results in this paper, we report on a factorial experiment design shown in Table \ref{tab:methods:parameters}, where we vary: 1) the regularization type, 2) the regularization strength ($\omega$), 3) the number of latent unroll steps ($K$), and 4) the size of the latent representation ($L = |\latents|$). Of course, our main interest is in the ability of the regularizations to influence performance. All experiments were run on the CPU. The hyperparameter analysis experiment was run asynchronously on a computing cluster using 24 threads at 2GHz. %All MountainCar runs were run sequentially on a laptop with a 9th generation i7 CPU. 
On average it took about half a day to train an agent on any particular environment. The complete experiments depicted take about one week time to complete (after the separate lengthy tuning phase of the other hyperparameters).  




